Are international happiness rankings reliable?

Global comparisons of wellbeing increasingly rely on survey questions that ask respondents to evaluate their lives, most commonly in the form of "life satisfaction" and "Cantril ladder" items. These measures underpin international rankings such as the World Happiness Report and inform policy initiatives worldwide, yet their comparability has not been established with contemporary global data. Using the Gallup World Poll, Global Flourishing Study, and World Values Survey, I show that the two question formats yield divergent distributions, rankings, and response patterns that vary across countries and surveys, defying simple explanations. To explore differences in respondents' cognitive interpretations, I compare regression coefficients from the Global Flourishing Study, analyzing how each question wording relates to life circumstances. While international rankings of wellbeing are unstable, the scientific study of the determinants of life evaluations appears more robust. Together, the findings underscore the need for a renewed research agenda on critical limitations to cross-country comparability of wellbeing.

==> rankpapertexstrings.tex <==
\newcommand\GWPindivCorrLSCL{0.63\xspace
} % 2025-08-21
\newcommand\GFSindivCorrLSCL{0.56\xspace
} % 2025-08-21
\newcommand\yearRangeCLGWP{2006--2022\xspace
} % 2025-09-02
\newcommand\yearRangeCLGWPTwentyOneTwentyTwoGFScountries{2021--2022\xspace
} % 2025-09-02
\newcommand\yearRangeCLGWPmatchedtoWVS{2006--2022\xspace
} % 2025-09-02
\newcommand\yearRangeLSWVSmatchedtoGFS{2001--2022\xspace
} % 2025-09-02
\newcommand\yearRangeLSWVSmatchedtoGWPLSwithinfouryears{2005--2013\xspace
} % 2025-09-02
\newcommand\yearRangeCLGFS{2023\xspace
} % 2025-09-02
\newcommand\yearRangeCLGWPTwentyOneTwentyTwo{2021--2022\xspace
} % 2025-09-02
\newcommand\yearRangeCLGWPmatchedtoLS{2007--2010\xspace
} % 2025-09-02
\newcommand\yearRangeLSGFS{2023\xspace
} % 2025-09-02
\newcommand\yearRangeLSGWP{2007--2010\xspace
} % 2025-09-02
\newcommand\yearRangeLSWVSmatchedtoGWP{2006--2022\xspace
} % 2025-09-02
\newcommand\yearRangeLSWVSmatchedtoGWPLS{1996--2022\xspace
} % 2025-09-02
\newcommand\yearRangeLSGWPGFScountries{2007--2010\xspace
} % 2025-09-02
\newcommand\GWPindivCorrLSCLGFScountries{0.62\xspace
} % 2025-08-21

